Nothing But Geometric Constraints: A Model-Free Method for Articulated Object Pose Estimation

We propose an unsupervised vision-based system to estimate the joint configurations of the robot arm from a sequence of RGB or RGB-D images without knowing the model a priori, and then adapt it to the task of category-independent articulated object pose estimation. We combine a classical geometric formulation with deep learning and extend the use of epipolar constraint to multi-rigid-body systems to solve this task. Given a video sequence, the optical flow is estimated to get the pixel-wise dense correspondences. After that, the 6D pose is computed by a modified PnP algorithm. The key idea is to leverage the geometric constraints and the constraint between multiple frames. Furthermore, we build a synthetic dataset with different kinds of robots and multi-joint articulated objects for the research of vision-based robot control and robotic vision. We demonstrate the effectiveness of our method on three benchmark datasets and show that our method achieves higher accuracy than the state-of-the-art supervised methods in estimating joint angles of robot arms and articulated objects.

==> intro_v0.tex <==
High-accuracy sensor-based robotic arms are increasingly used in manufacturing, transport, and surgery. With the help of sensors, a robot can know accurate configuration of each joint and then uses it for close-loop control or reinforcement learning-based control \cite{andrychowicz2020learning}. But those sensors are not always available, especially for low-cost domestic used robotic arms \cite{zuo2019craves}, dexterous manipulations \cite{hang2019hand}, and robots works in special environments \cite{ortenzi2016vision}. It is also a common problem in multi-robot systems, in which robots operate in a shared workspace while each of them has no access to the joint encoder of other robots \cite{leitner2012transferring}. Therefore, robot pose estimation is indispensable to allow robots for broader use. 

To solve this problem, researchers proposed many methods.  However, existing methods either use fiducial markers \cite{ortenzi2016vision} to track the motion or require exact CAD models \cite{bohg2014robot,widmaier2016robot,ortenzi2016vision}, or need large annotated datasets \cite{zhou20193d,ma2020edge,miseikis2018multi,gulde2018ropose,lambrecht2019towards}
of a certain robot for training to detect the 2D keypoints, which severely restrict the use of these methods. 

%We argue that a generic, agile, robust, and low-cost robot pose estimation system can be achieved by well utilizing the vision information. Meanwhile, notice that the robot arm is a kind of complicated articulated object, so this system should be easy to be extended to the task of articulated object pose estimation, which is another highly relevant topic in building home service robots.

It may be easy to get a CAD model for a robot arm, but if we consider a more general task, i.e. articulated object pose estimation (the robot arm can be seen as a kind of complicated articulated object),  current methods still need exact CAD models \cite{michel2015pose,ye2014real,desingh2019factored,pavlasek2020parts} or category-level shape representation \cite{abbatematteo2019learning,yi2018deep,li2020category}, which is much more difficult to build considering the great varieties of articulated objects in our daily environment. We argue that a model-free, agile, robust, and low-cost articulated object pose estimation system can be achieved by well utilizing the vision information.

%This is going to confuse people -- you're not really computing the 6 DOF pose of "the robot". In robotics, we talk about the "configuration" of a robot as the set of values that determine the 6DOF pose of all of the joints. I'd recommend you use the term "configuration" here and/or define the pose of the robot as the configuration of its joints explicitly. It is unfortunate that people talk about the pose of a body as the configuration of the limbs, but we can't change that ..

In this paper, we proposed an unsupervised vision-based method, namely GC-Pose, to estimated the 3D pose of any kinds of robot arms or articulated objects from a video sequence. Mathematically, given a single-view video sequence $\mathcal{I}$ of a robot, a vision model $\mathcal{M}:\mathbf{P}=h(\mathcal{I},\bm{\theta})$ is proposed to estimate the 3D pose of each rigid part without using the CAD model or training on annotated data. Specifically, we are particularly interested in the joint configurations $\mathbf{q}$ of the robot since the pose of a robot is well-determined given the joint configurations. Considering that in reality, robot arms start moving from the home position, which is unique and known for most kinds of robot arms, we can assume that the first frame of the given video sequence shows the home pose/position of the robot, then the problem can be simplified into estimating the change of the joint configuration in the give video sequences. An overview is shown in Figure \ref{fig:teaser}. 

To achieve this goal, several major challenges need to be addressed: \textbf{First}, different from most 3D pose estimation algorithms which need to know the exact object CAD model \cite{li2018deepim,brachmann2014learning,desingh2019factored} or shared representation for different instances within a given category \cite{wang2019normalized,li2020category}, we want to estimate the joint configurations of robot or articulated objects directly from the input video sequences without knowing the CAD model or category a priori. \textbf{Second}, real-world robot arms and articulated objects usually have low-textured and reflective surfaces, which makes it harder to extract information from video sequences. \textbf{Third}, in contrast to a rigid object, a robot arm is composed of several connected rigid parts, and joint constraints hold for every adjacent parts, leading to a higher degree of freedom (DoF) with physical constraints. \textbf{Lastly}, a robot arm may have a complicated motion pattern, including rotating by the axis direction parallel to the screen, which leads to ambiguity and uncertainty, and self-occlusion, which leads to results fluctuation and large errors.

%To solve the challenge caused by not using the CAD model, an optical flow-based algorithm for robot arm pose estimation, namely GC-Pose, is proposed. Given a video sequence of a moving robot arm, the optical flow is estimated to get the pixel-wise dense correspondences. Then we use RANSAC\cite{fischler1981random} and the EM algorithm\cite{dempster1977maximum} to split different moving parts. After that, for each moving part, we introduce a modified Perspective-$n$-Point (P$n$P)\cite{lepetit2009epnp} algorithm to compute the change of the 3D pose from 2D correspondences. Finally, the joint configuration of each moving part is computed from the 3D pose we estimated.

To solve the challenge caused by not using the CAD model, an optical flow-based algorithm is proposed to estimate the relative pose of the articulated objects. When humans interact with the environment, we do not need to know the exact pose. Instead, we learn the relative pose or relative motion of the objects during the interaction. We borrow from this idea and estimate the change of the pose from a given video sequence instead of directly estimating the absolute pose. Then we compute the joint configuration of each moving part from the related pose we estimated.

To solve the challenge caused by low-textured surfaces, we extend the use of epipolar constraint to multi-rigid-body systems. This constraint holds since each moving part of a robot is a rigid body, and the optical flow for this part should be satisfied with one 3D transformation. Mathematically, for each pixel $\mathbf{p}^\alpha$ belongs to the rigid body $\alpha$, the following equation holds: $\mathbf{p}^\alpha+\mathbf{F}(\mathbf{p}^\alpha)=\mathbf{T}(\mathbf{p}^\alpha;\mathbf{R}^\alpha,\mathbf{t}^\alpha)$, where $\mathbf{F}(\mathbf{p}^\alpha)$ denotes the optical flow,  $\mathbf{R}^\alpha$ and $\mathbf{t}^\alpha$ denote the rotation matrix and transformation matrix in 3D space. Considering that $\mathbf{R}^\alpha$ and $\mathbf{t}^\alpha$ only have 6 DoF, these constraints provide us each rigid body optical flow estimation for a rigid body with only 6 DOF instead of optical flow for each pixel. Thus it helps lessen the problem caused by the low-textured area of a rigid body.

To solve the ambiguity and fluctuation caused by complicated motion patterns, we use the geometric constraints between multiple frames. We reconstruct the 3D shape of the moving robot arm from these frames, then use bundle adjustment to optimize the joint configurations we estimate. In this paper, we use the 3D point cloud model to represent the shapes. Since we don't aim to generate an exact 3D model, we can use either estimated depth or depth from the RGB-D camera to reconstruct the 3D point cloud model. Our experiments show that even if the point cloud model is noisy and can only represent a small area of the robot arm, it still can be used to optimize the joint configurations and improve the estimation accuracy on robot arms with complicated motion patterns.

We evaluated the performance of our system by conducting three sets of experiments on three benchmark datasets. To better evaluate our system, we also developed a dataset of different kinds of robots and multi-joint articulated objects. We compared our system with CRAVES\cite{zuo2019craves}, a state-of-the-art (SOTA) robot pose estimation algorithm, and ScrewNet\cite{jain2020screwnet}, a SOTA articulation model estimation method. The experimental results show that our system outperforms these supervised pose estimation methods. Then we perform ablation studies on our synthetic dataset. Our experiments demonstrate that leveraging the geometric constraints of the rigid body and constraints between multiple frames helps handle the low-textured area and complicated motion pattern, which leads to improved performance in unsupervised, model-free articulated pose estimation.
% the simulated robot arm data set provided by Zuo, the simulated articulated objects dataset provided by Abbatematteo, and the recently proposed PartNet-Mobility dataset.

In summary, our contributions are:
\begin{itemize}[topsep=0pt,itemsep=0pt,parsep=0pt]
\item We propose a model-free pose estimation method (GC-Pose), which can estimate the joint configurations of robot arms or articulated objects from a video sequence without CAD model or annotated dataset.
\item We demonstrate that the extended epipolar constraint can help handle the low-textured area of a rigid body.
\item We develop a benchmark dataset of different kinds of robots and multi-joint articulated objects with various labels for vision-based robot control, robotic vision, and robotic manipulation tasks.
%Compared with the existing simulated articulated objects dataset, it is more realistic due to the changeable appearance, and meanwhile, it has more complicated poses and variable joints. 
\end{itemize}
 
\begin{comment}
Contribution:

1) a system to estimate robotic arm pose without CAD model and labeling.

2) epipolar flow to handle low texture area

3) a dataset for benchmark

4) a vision based control system

5) More realistic data, control the robot arm appearance?

6) use dataset to diagnosis model robustness

7) rigid body pose estimation from optical flow ? 
\end{comment}

==> intro_v1.tex <==
Articulated object pose estimation is an important task which attracts more attentions over time. 
It can be applied to robotic arm pose estimation.
Articulated object pose estimation is important for an AI to interact with the world and has great value for applications.
safety backup, robot collaboration, low-cost robot control, robot manipulation. Solving this problem can greatly increase the ability for a robot to interact with the real world.

Most pose estimation method is instance-level or category-level, which means the model needs to be trained with data of the same instance or from the same category.  category-level\cite{xiaolong}. SMPL.
This limits the applications, there are various kinds of objects. It is difficult to observe instance beforehand, and the category level sometimes has dramatic intra-class variation。
When we saw a new articulated object, we can discover parts of the objects by observing a video.
This makes us wonder can we estimate articulated object pose without the shape knowledge of the object? Without knowing the object shape, can we achieve similar performance to supervisedly trained models.
% Fit a model into the image, video? The SE-net, the talk paper, the SLAM paper.

% Can we compare with previous model free approach? Can we say previous model-free is not popular?
In this paper, we propose a model-free approach. 
The articulated structure is discovered from a video sequence. Our model discover parts of objects from dense correspondence between frames. 
Parts of the object can be discovered from consective frames by clustering the motion vectors.
Different from supervised trained model, which can give the absolute angle, our method can only give the relative transformation between frames, then the absolute angle can be accumulated over frames.
Part discovery can be estimated from videos.

% The challenges for a robust articulated pose estimation.
% a robot arm may have a complicated motion pattern, including rotating by the axis direction parallel to the screen, which leads to ambiguity and uncertainty, and self-occlusion, which leads to results fluctuation and large errors.
% real-world robot arms and articulated objects usually have low-textured and reflective surfaces, which makes it harder to extract information from video sequences.

Challenges of articulated object estimation makes previous models suffer. Factors are self-occlusion, low-texture area, refection, ambiguous pose, small parts.
Previously, model-free models suffer.
The dense correspondence is noisy, especially for objects with low texture area, such a furniture or a robot arm. 
So we apply epipolar constraint to get a rigid flow. 
Since we know the object is composed with articulated parts, we can use the epipolar constraint to refine the flow.
% Explain the epipolar concept.
Bundle adjustment to fix errors in local estimation.


Experiment shows our method can achieve similar performance compared with supervisely trained model and largely surpass existing model-free models. We also use synthetic data to perform extensive abalation study to understand the properties of our model.
We evaluated the performance of our system by conducting three sets of experiments on three benchmark datasets. 
To better evaluate our system, we also developed a dataset of different kinds of robots and multi-joint articulated objects. 
ScrewNet\cite{jain2020screwnet}, a SOTA articulation model estimation method.
We compared our system with CRAVES\cite{zuo2019craves}, a state-of-the-art (SOTA) supervised robot pose estimation algorithm.
The experimental results show that our system outperforms these supervised pose estimation methods. 
Our synthetic data helps us to study the impact of our modules by controlling image appearance and generating intermediate ground truth.
Then we perform ablation studies on our synthetic dataset. 
Our experiments demonstrate that leveraging the geometric constraints of the rigid body and constraints between multiple frames helps handle the low-textured area and complicated motion pattern, which leads to improved performance in unsupervised, model-free articulated pose estimation.


In summary, our contributions are:
\begin{itemize}[topsep=0pt,itemsep=0pt,parsep=0pt]
\item We propose a model-free pose estimation method (GC-Pose), which can estimate the joint configurations of robot arms or articulated objects from a video sequence without CAD model or annotated dataset.
\item We demonstrate that the extended epipolar constraint can help handle the low-textured area of a rigid body.
% \item We develop a benchmark dataset of different kinds of robots and multi-joint articulated objects with various labels for vision-based robot control, robotic vision, and robotic manipulation tasks.
\item Extensive experiments show the effectiveness of our method. We also developed a synthetic dataset to analyze the property of our model.
\end{itemize}

% Technical novelty. 1. epipolar for better flow, 2. 

% Define the problem?
% Why this problem is important?
% Why model free?
% Why other can not achieve model free and we can?
% Why our model is better?
% Articulated object pose estimation is important? safety, robot collaboration, low-cost robot, scene manipulation.
% Why model free is important?
% Why we can do model free? Why others can not achieve model free?
% Method, which input to the model is required?
